Spectral Properties and Stability of Self-Similar Wave Maps

In this thesis the Cauchy problem and in particular the question of singularity formation for co--rotational wave maps from 3+1 Minkowski space to the three--sphere $S^3$ is studied. Numerics indicate that self--similar solutions of this model play a crucial role in dynamical time evolution. In particular, it is conjectured that a certain solution $f_0$ defines a universal blow up pattern in the sense that the future development of a large set of generic blow up initial data approaches $f_0$. Thus, singularity formation is closely related to stability properties of self--similar solutions. In this work, the problem of linear stability is studied by functional analytic methods. In particular, a complete spectral analysis of the perturbation operators is given and well--posedness of the linearized Cauchy problem is proved by means of semigroup theory and, alternatively, the functional calculus for self--adjoint operators. These results lead to growth estimates which provide information on the stability of self--similar wave maps. Finally, convergence properties of $f_n$ for large $n$ and the spectra of the corresponding perturbation operators are investigated. The thesis is intended to be self--contained as far as possible, i.e. all the mathematical requirements are carefully introduced, including proofs for many results which could be found elsewhere.

==> specln/opth.tex <==
\section{Operator Theory}
\label{opth_sec}
In order to define and study the operator $A_\infty$ it is useful to introduce
some more general theory. 
Therefore, we will discuss a criterion for essential self--adjointness for a
symmetric operator and review some aspects of Sturm--Liouville theory.
We will also give proofs for most of the results stated below 
since they are very instructive.
For more detailed expositions see e.g. 
\cite{Kato1980}, \cite{Yosida1980}, \cite{Naimark1968} and
\cite{Teschl2007}.

\subsection{Essential Self--Adjointness}
Once we are given a symmetric operator $A_0: \Dom{A_0} \subset H \to H$ on a
Hilbert space $H$ we can ask the question whether there exist self--adjoint
extensions of $A_0$.
As we have seen, self--adjointness is a very strong property and hence it is
desireable to work with self--adjoint operators since they are convenient to
handle.
Thus, it is important to find an easy criterion whether a given symmetric
operator admits self--adjoint extensions.
A second issue is the question of uniqueness of such an extension.
There exists a well--known general theory on this subject and we will state some
results.

Recall that a symmetric operator $A_0$ is called essentially self--adjoint 
if its
closure $\overline{A_0}$ is self--adjoint.
This is the simplest case of a self--adjoint extension and it is automatically
unique: Another self--adjoint extension $A_1$ has to be an extension of
$\overline{A_0}$ since $A_1$ is closed and $\overline{A_0}$ is the smallest
closed extension of $A_0$. However, self--adjoint operators do not have proper
symmetric extensions and hence, $A_1=\overline{A_0}$.
Thus, it is desireable to have an easy criterion for a symmetric operator to be
essentially self--adjoint.
To this end we prove two simple results concerning symmetric operators.

\begin{lemma}
\label{Ainf_lem_symmsa}
Let $A: \Dom{A} \subset H \to H$ be a symmetric operator on a Hilbert space $H$.
If there exists a $\lambda \in \mathbb{C}$ such that
$\mathrm{im}(\lambda-A)=\mathrm{im}(\overline{\lambda}-A)=H$ then $A$ is
self--adjoint.
\end{lemma}

\begin{proof}
Let $v \in \Dom{A^*}$, i.e. there exists a $w \in H$ such that
$(Au|v)_H=(u|w)_H$ for all $u \in \Dom{A}$.
We have to show that $v \in \Dom{A}$.
Since $\mathrm{im}(\overline{\lambda}-A)=H$ there exists a $\tilde{v} \in
\Dom{A}$ such that $\overline{\lambda}-A)\tilde{v}=\overline{\lambda}v-w$.
We calculate
$$
((\lambda-A)u|v)_H=(u|\overline{\lambda}v-w)_H=
(u|(\overline{\lambda}-A)\tilde{v})_H=((\lambda-A)u|\tilde{v})_H $$
for all $u \in \Dom{A}$ by the symmetry of $A$.
However, since $\lambda-A$ is surjective we conclude $v=\tilde{v} \in \Dom{A}$.
Hence, we have shown that $A^* \subset A$ which implies $A^*=A$ since $A \subset
A^*$ by assumption.
\end{proof}

\begin{lemma}
\label{Ainf_lem_iminc}
Let $A: \Dom{A} \subset H \to H$ be a closeable linear operator on a 
Hilbert space $H$. Then, we have the inclusion 
$\mathrm{im}\overline{A} \subset \overline{\mathrm{im}A}$.
\end{lemma}

\begin{proof}
Let $f \in \mathrm{im}\overline{A}$, i.e. there exists a $u \in
\Dom{\overline{A}}$ such that $\overline{A}u=f$.
By the definition of the closure it follows that there exists a sequence 
$(u_j) \subset \Dom{A}$ such that $u_j \to u$ in $H$ and $A u_j \to
\overline{A}u$ in $H$.
Define $f_j:=Au_j$.
Then, $(f_j) \subset \mathrm{im}A$ and $f_j \to f$ in $H$.
Hence, $f \in \overline{\mathrm{im}A}$.
\end{proof}

\begin{lemma}
\label{Ainf_lem_symmsur}
Let $A: \Dom{A} \subset H \to H$ be a symmetric operator on a Hilbert space $H$.
Then, $\mathrm{im}(\lambda-\overline{A})=\overline{\mathrm{im} (\lambda-A)}$ for
any $\lambda \in \mathbb{C}\backslash \mathbb{R}$.
\end{lemma}

\begin{proof}
As a symmetric operator, $A$ is closeable and hence, lemma \ref{Ainf_lem_iminc}
yields the inclusion $\mathrm{im}(\lambda-\overline{A}) \subset 
\overline{\mathrm{im} (\lambda-A)}$.

We write $\lambda=\kappa + i\omega$ where $\kappa,\omega \in \mathbb{R}$ and
$\omega \not=0$ by assumption.
Using the symmetry of $\overline{A}$ ($A \subset A^*$ implies $\overline{A}
\subset A^*$) we readily estimate
\begin{multline}
\label{Ainf_est_improof}
\|(\lambda-\overline{A})u\|_H^2
=\|(\kappa-\overline{A})u\|_H^2+2 \Re ((\kappa-\overline{A})u|i\omega u)_H +
\|i\omega u\|_H^2 \\
=\|(\kappa-\overline{A})u\|_H^2+\omega^2 \|u\|_H \geq \omega^2 \|u\|_H^2
\end{multline}
for any $u \in \Dom{\overline{A}}$.
Now let $f \in \overline{\mathrm{im}(\lambda-A)}$, i.e. there exists a 
sequence
$(f_j) \subset \mathrm{im}(\lambda-A)$ such that $f_j \to f$ in $H$.
Hence, there exist $u_j \in \Dom{A}$ such that $(\lambda-A)u_j=f_j$.
Furthermore, we have $\|u_j-u\|_H \leq \omega \|f_j-f\|_H \to 0$ by estimate
(\ref{Ainf_est_improof}).
This shows $u_j \to u$ in $H$ and from the closedness of $\lambda-\overline{A}$
we conclude that $u \in \Dom{\overline{A}}$ and $(\lambda-\overline{A})u=f$ which implies
$f \in \mathrm{im}(\lambda-\overline{A})$.
Thus, we have shown $\overline{\mathrm{im}(\lambda-A)} \subset
\mathrm{im}(\lambda-\overline{A})$ which finishes the proof.
\end{proof}

Now we are ready to prove a criterion for essential self--adjointness of a
symmetric operator.
To this end we first note a simple relation between 
$\ker A^*$ and $\mathrm{im}A$.

\begin{lemma}
\label{Ainf_lem_kerim}
Let $A: \Dom{A} \subset H \to H$ be a densely defined linear operator on a
Hilbert space $H$. Then, $\ker A^*=(\mathrm{im}A)^\perp$.
\end{lemma}

\begin{proof}
$\Dom{A}$ is dense and hence, the adjoint $A^*$ is defined.
Let $v \in \Dom{A^*}$.
Then, we have
$v \in \ker A^*$ $\Leftrightarrow$ $(u|A^*v)_H=0$ $\forall u \in \Dom{A}$
$\Leftrightarrow$ $(Au|v)_H=0$ $\forall u \in \Dom{A}$ $\Leftrightarrow$ $v \in
(\mathrm{im} A)^\perp$. 
\end{proof}

\begin{lemma}
\label{Ainf_lem_esssa}
Let $A: \Dom{A} \subset H \to H$ be a symmetric operator on a Hilbert space.
$A$ is essentially self--adjoint if and only if there exists a $\lambda \in
\mathbb{C} \backslash \mathbb{R}$ such that
$\ker(\lambda-A^*)=\ker(\overline{\lambda}-A^*)=\{0\}$.
\end{lemma}

\begin{proof}
By lemma \ref{Ainf_lem_kerim} we have
$$ \{0\}=\ker(\overline{\lambda}-A^*)=\ker(\lambda-A)^*
=(\im(\lambda-A))^\perp $$
and thus, $\overline{\im(\lambda-A)}=H$.
However, lemma \ref{Ainf_lem_symmsur} tells us that
$H=\overline{\im(\lambda-A)}=\im(\lambda-\overline{A})$.
The same calculation with $\overline{\lambda}$ substituted by $\lambda$ yields
$\im(\lambda-\overline{A})=H$.
Invoking lemma \ref{Ainf_lem_symmsa} we conclude that $\overline{A}$ is
self--adjoint and hence, $A$ is essentially self--adjoint.

Conversely, if $A$ is self--adjoint then clearly
$\ker(\lambda-A^*)=\ker(\overline{\lambda}-A^*)=\{0\}$ for any $\lambda \in
\mathbb{C} \backslash \mathbb{R}$ since $\sigma(A^*)=\sigma(A) \subset
\mathbb{R}$. 
\end{proof}

We define the \emph{defect indices} $d_+(A), d_-(A)$ of a symmetric
operator $A$ on a Hilbert space by $d_\pm(A):=\dim \ker(\pm i - A^*)$.
Thus, lemma \ref{Ainf_lem_esssa} tells us that the operator $A$ is essentially
self--adjoint if its defect indices are equal to zero.
However, one can show (cf. \cite{Kato1980}) that the numbers $\dim
\ker(\lambda-A^*)$ are constant on the upper and lower half--plane and hence, we
have the result that $A$ is essentially self--adjoint if and only if
$d_+(A)=d_-(A)=0$.

\subsection{Sturm--Liouville Operators}

\paragraph{Absolutely continuous functions}
We introduce a new function space which turns out to be useful in connection
with ordinary differential operators.
Let $u: [a,b] \to \mathbb{C}$.
Then, $u \in AC[a,b]$ if there exists a function $v \in L^1(a,b)$ and a 
$c \in (a,b)$ such that $u(x)-u(c)=\int_c^x v(s)ds$ for all $x \in [a,b]$.
In particular, it follows that $u$ is continuous and possesses a
weak derivative given by $v$. 
Clearly, $AC[a,b]$ is a vector space and it is called the space of
\emph{absolutely continuous functions}.
As usual, the local version $AC_{\mathrm{loc}}(a,b)$ is defined as
$AC_{\mathrm{loc}}(a,b):=\{u \in AC[c,d]: [c,d] \subset (a,b)\}$.

\paragraph{Sturm--Liouville operators}
A Sturm--Liouville operator is generated by a formal differential 
expression $\alpha$
of the form
$$ \alpha u:=\frac{1}{w}\left (-(pu')'+qu \right ) $$
where $p,q: (a,b) \to \mathbb{R}$, $1/p,q \in L^1_{\mathrm{loc}}(a,b)$ and $w$
is a weight function.

Formal integration by parts yields the \emph{Green's formula}
\begin{equation}
\label{Ainf_eq_Green} \int_c^d (\alpha u)(x)\overline{v(x)}w(x)dx=[u,v]_p(d)-[u,v]_p(c)+\int_c^d
u(x)\overline{(\alpha v)(x)}w(x)dx 
\end{equation}
for any $[c,d] \subset (a,b)$ where
$[u,v]_p(x):=u(x)\overline{(pv')(x)}-(pu')(x)\overline{v(x)}$. 

\paragraph{The initial value problem}
Consider the equation 
$$ (pu')'+qu=\lambda w u $$
on $(a,b) \subset \mathbb{R}$ for a complex parameter $\lambda$.
The assumptions on $p,q$ are sufficient to guarantee 
existence and uniqueness of
the initial value problem.
More precise, we have the following theorem.

\begin{theorem}
\label{opth_thm_ivp}
Let $c \in (a,b)$ and $\xi,\eta \in \mathbb{C}$.
Then, there exists a unique function $u(\cdot, \lambda) \in
AC_\mathrm{loc}(a,b)$ with $pu'(\cdot,\lambda) \in AC_\mathrm{loc}(a,b)$ 
such that
$(pu')'+qu=\lambda w u$ and $u(c, \lambda)=\xi$, $(pu')(c, \lambda)=\eta$.
Moreover, the function $u(x, \cdot)$ is holomorphic on $\mathbb{C}$ for any $x
\in (a,b)$.
\end{theorem}

The proof is similar to the classic Picard--Lindel\"of theorem and can be
found e.g. in \cite{Naimark1968}.

\paragraph{The maximal operator}
We set $H:=L^2_w(a,b)$ and define the \emph{maximal operator} $A_1: \Dom{A_1}
\subset H \to H$ associated
to $\alpha$ by 
$$ \Dom{A_1}:=\{u \in H: u,pu' \in AC_\mathrm{loc}(a,b), \alpha u \in
H\} $$
and $A_1u:=\alpha u$ for $u \in \Dom{A_1}$.
Note that functions $u$ in $\Dom{A_1}$ satisfy the minimal requirements to give
sense to $\alpha u$ and to guarantee $u \in H$ as well as $\alpha u \in H$.
That is why $A_1$ is called the maximal operator.
Note further that $u,v \in \Dom{A_1}$ implies the existence of 
$$ [u,v]_p(a):=\lim_{x \to a+}[u,v]_p(x) \mbox{ and }[u,v]_p(b):=\lim_{x \to
b-}[u,v]_p(x) $$
as follows from the Green's formula eq. (\ref{Ainf_eq_Green}).

\paragraph{Endpoint classification}
The endpoint $a$ of the interval $(a,b)$ is classified as follows.
\begin{itemize}
\item The endpoint $a$ is said to be \emph{regular} if $a>-\infty$ and 
there exists a $c \in
(a,b)$ such that $1/p,q,w \in L^1(a,c)$.
\item $a$ is said to be in the \emph{limit--circle} case if there exist $u,v \in
\Dom{A_1}$ such that $[u,v]_p(a) \not= 0$.
\item Finally, $a$ is said to be in the \emph{limit--point} case if
$[u,v]_p(a)=0$ for all $u,v \in \Dom{A_1}$.
\end{itemize}
The same classification is applied to $b$.

Without proof we note the important fact that there exists a close connection
between endpoint classification and integrability of solutions of the equation
$\alpha u=0$.
For instance, $a$ is limit--point if and only if there exists at least one
solution $u$ of $\alpha u=0$ which does not belong to $H$ near $a$
\footnote{One says that the function $u$ belongs to $L^2_w(a,b)$ near $a$ 
if there exists a $c \in
(a,b)$ such that $u|_{(a,c)} \in L^2_w(a,c)$.}.
This is essentially a consequence of the variations of constants formula.

\paragraph{The minimal operator}
The \emph{minimal operator} $A_0: \Dom{A_0} \subset H \to H$ 
associated to $\alpha$ is defined by
$$ \Dom{A_0}:=\{u \in \Dom{A_1}: [u,v]_p(a)=[u,v]_p(b)=0 \mbox{ for all
} v \in \Dom{A_1}\} $$
and $A_0u:=\alpha u$ for $u \in \Dom{A_0}$.
Obviously, we have $A_0 \subset A_1$.
Furthermore, $(A_0u|v)_H=(u|A_1v)_H$ for all $u \in \Dom{A_0}$ and $v \in
\Dom{A_1}$, i.e. the operators $A_0$ and $A_1$ are adjoint to each other.
This observation leads to the first easy relationship between $A_0$ and $A_1$.

\begin{lemma}
\label{opth_lem_imsubker}
We have the inclusion $\im{A_0} \subset (\ker{A_1})^\perp$.
\end{lemma}

\begin{proof}
Let $f \in \im{A_0}$, i.e. there exists a $u \in \Dom{A_0}$ such that $A_0u=f$.
Choose any $v \in \ker{A_1}$.
Then, since $A_0$ and $A_1$ are adjoint to each other, we have 
$(f|v)_H=(A_0u|v)_H=(u|A_1v)_H=0$.
\end{proof}

\subsection{Regular Sturm--Liouville Operators}
We prove some properties of $A_0$ and $A_1$.
However, it is easier to consider the regular case first.
Thus, we assume that
both endpoints $a$ and $b$ are regular, i.e. $1/p,q,w \in L^1(a,b)$.
The regular case allows major simplifications.
First of all, any $u \in C[a,b]$ belongs to $H=L^2_w(a,b)$ thanks to the
inequality $\int_a^b |u(x)|^2w(x)dx \leq \||u|^2\|_{C[a,b]}
\|w\|_{L^1(a,b)}<\infty$
and, secondly, the initial value problem can be uniquely solved at the
endpoints, i.e. the point $c$ in theorem \ref{opth_thm_ivp} can be chosen to be
$a$ or $b$.
Moreover, any solution $u$ of $A_1 u=0$ satisfies $u,pu' \in AC[a,b]$.

\paragraph{Relation between $\im{A_0}$ and $\ker{A_1}$}

\begin{lemma}
\label{opth_lem_A1surj}
Let $f \in H$. Then, we can find a function $u \in \Dom{A_1}$ satisfying
$u(a)=(pu')(a)=0$ and $A_1u=f$. In particular, $A_1$ is surjective.
\end{lemma}

\begin{proof}
Let $f \in H$.
Since $A_1$ is regular we can find two linearly independent functions $u_1, u_2
\in \Dom{A_1}$ satisfying $A_1u_j=0$ and $u_j,pu_j' \in AC[a,b]$ for $j=1,2$.
Moreover, $[u_1,u_2]_p(x)$ is a constant $\not= 0$ 
as follows from the Green's formula eq.
(\ref{Ainf_eq_Green}) and thus, by normalization we can assume that
$[u_1,u_2]_p(x)=1$. 
We set 
$$ u(x):=u_1(x)\int_a^x u_2(s) f(s) w(s)ds-u_2(x)\int_a^x u_1(s) f(s) w(s)ds. $$
The involved integrals exist thanks to the inequality 
\begin{multline*}
\int_a^b u_j(x) f(x) w(x)dx \leq 
\left ( \int_a^b |u_j(x)|^2 w(x)dx \right )^{1/2}
\|f\|_H \\
\leq \left ( \||u_j|^2\|_{C[a,b]}\|w\|_{L^1(a,b)} \right )^{1/2} \|f\|_H^2<\infty. 
\end{multline*}
A direct computation reveals $u,pu' \in AC[a,b]$, $u(a)=(pu')(a)=0$
and $A_1u=f$.
\end{proof}

Now we are ready to prove the converse statement to lemma
\ref{opth_lem_imsubker}.

\begin{lemma}
\label{opth_lem_kersubim}
Let $f \in (\ker{A_1})^\perp$. Then, $f \in \im{A_0}$.
\end{lemma}

\begin{proof}
Let $f \in (\ker{A_1})^\perp$. According to lemma \ref{opth_lem_A1surj} we can
find a $u \in \Dom{A_1}$ such that $u(a)=(pu')(a)=0$ and $A_1 u =f$.
Let $u_1,u_2 \in \ker{A_1}$ satisfying $u_1(b)=(pu'_2)(b)=0$ and
$u_2(b)=(pu'_1)(b)=1$.
Such functions exist thanks to theorem \ref{opth_thm_ivp} and the regularity
of $A_1$. 
Invoking Green's formula eq. (\ref{Ainf_eq_Green}) we calculate
$$ 0=(f|u_j)_H=(A_1u|u_j)_H=[u,u_j]_p(b)-[u,u_j]_p(a)
+(u|A_1u_j)_H=[u,u_j]_p(b) $$
for $j=1,2$ which yields $u(b)=(pu')(b)=0$.
Thus, $u \in \Dom{A_0}$ and we have $A_0u=A_1u=f$ which shows that $f \in
\im{A_0}$.
\end{proof}

\begin{remark}
\label{opth_rem_imker}
Taking together lemmas \ref{opth_lem_imsubker} and \ref{opth_lem_kersubim} we
have proved that $\im{A_0}=(\ker{A_1})^\perp$. 
Note that the existence and uniqueness theorem \ref{opth_thm_ivp} implies that
$\ker{A_1}$ is two--dimensional and in particular, as a finite--dimensional
normed vector space, it is closed.
Thus, by taking the orthogonal complement, the relation
$\im{A_0}=(\ker{A_1})^\perp$ implies $(\im{A_0})^\perp=\ker{A_1}$.
\end{remark} 

\paragraph{Density of $\Dom{A_0}$}
Next we prove that $\Dom{A_0}$ is dense in $H$ which shows that $A_0$ and $A_1$
are densely defined.

\begin{lemma}
\label{opth_lem_A0dense}
The domain $\Dom{A_0}$ is dense in $H$.
\end{lemma}

\begin{proof}
It suffices to show that any element which is orthogonal to $\Dom{A_0}$ is zero.
Let $f \in \Dom{A_0}^\perp$, i.e. $(u|f)_H=0$ for all $u \in \Dom{A_0}$.
Invoking lemma \ref{opth_lem_A1surj} we see that 
there exists a $v \in \Dom{A_1}$ such
that $A_1 v=f$.
Thus, we have
$0=(u|f)_H=(u|A_1v)_H=(A_0u|v)_H$
for all $u \in \Dom{A_0}$ which shows that $v \in (\im{A_0})^\perp$.
However, according to remark \ref{opth_rem_imker} we have
$(\im{A_0})^\perp=\ker{A_1}$ and thus, $v \in \ker{A_1}$ which yields
$0=A_1v=f$.
\end{proof}

\paragraph{The adjoints}
We calculate the adjoints of $A_0$ and $A_1$ (which are now known to exist since
$A_0$ and $A_1$ are densely defined).

\begin{lemma}
\label{opth_lem_adjA0}
The operator $A_1$ is the adjoint of $A_0$, i.e. $A_0^*=A_1$.
\end{lemma}

\begin{proof}
According to the Green's formula eq. (\ref{Ainf_eq_Green}) we know that
$(A_0u|v)_H=(u|A_1v)_H$ for all $u \in \Dom{A_0}$ and $v \in \Dom{A_1}$ which
means that $A_1 \subset A_0^*$.
Let $v \in \Dom{A_0^*}$, i.e. there exists an $f \in H$ such that
$(u|f)_H=(A_0u|v)_H$ for all $u \in \Dom{A_0}$.
However, since $A_1$ is surjective by lemma \ref{opth_lem_A1surj} there exists a
$\tilde{v} \in \Dom{A_1}$ such that $A_1 \tilde{v}=f$.
Hence, we have
$$ (A_0u|v)_H=(u|f)_H=(u|A_1 \tilde{v})_H=(A_0u|\tilde{v})_H $$
which shows that $(A_0u|v-\tilde{v})_H=0$.
We conclude that 
$v-\tilde{v} \in (\im{A_0})^\perp=\ker{A_1} \subset \Dom{A_1}$ (remark
\ref{opth_rem_imker}) and therefore, since $\tilde{v} \in \Dom{A_1}$,
we infer that $v \in \Dom{A_1}$.
Thus, we have shown that $A_0^* \subset A_1$ which finishes the proof.
\end{proof}

\begin{remark}
In particular it follows that $A_1$ is closed since it coincides with the
adjoint of a densely defined operator which is always closed.
\end{remark}

\begin{lemma}
\label{opth_lem_adjA1}
The operator $A_0$ is the adjoint of $A_1$, i.e. $A_1^*=A_0$.
\end{lemma}

\begin{proof}
Applying "$^*$" to the relation $A_1=A_0^*$ (lemma \ref{opth_lem_adjA0}) 
yields $A_1^*=A_0^{**} \supset A_0$.
Thus, it remains to show that $A_1^* \subset A_0$.
The relation $A_1 \supset A_0$ implies $A_1^* \subset A_0^*$ and we infer $A_1^*
\subset A_1$.
Let $v \in \Dom{A_1^*} \subset \Dom{A_1}$.
By definition of the adjoint we have $(A_1u|v)_H=(u|A_1^*v)_H=(u|A_1v)_H$ for
all $u \in \Dom{A_1}$.
On the other hand, by the Green's formula eq. (\ref{Ainf_eq_Green}), we have
$(A_1u|v)_H=[u,v]_p(b)-[u,v]_p(a)+(u|A_1v)_H$ for all $u \in \Dom{A_1}$ 
and thus, $[u,v]_p(b)-[u,v]_p(a)=0$ for all $u \in \Dom{A_1}$.
However, since $A_1$ is regular we can choose $u(a),(pu')(a),u(b),(pu')(b)$
arbitrarily and we conclude that $v(a)=(pv')(a)=v(b)=(pv')(b)=0$ 
which shows that $v
\in \Dom{A_0}$ and therefore, $A_1^* \subset A_0$.
\end{proof}

\begin{remark}
Again, it follows that $A_0$ is closed.
\end{remark}

\paragraph{A special case}
The operator $A_0$ is symmetric but it is not self--ajoint since $A_0^*=A_1
\not=A_0$.
Thus, possible self--adjoint extensions of $A_0$ 
lie between $A_0$ and $A_0^*=A_1$.
We give a simple example.
Let $\Dom{A}:=\{u \in \Dom{A_1}: u(a)=u(b)=0\}$ and $Au:=\alpha u$ for $u \in
\Dom{A}$.
Then, $A_0 \subset A \subset A_1$.
We claim that $A$ is self--adjoint. 
 
\begin{lemma}
The operator $A$ is self--adjoint.
\end{lemma}

\begin{proof}
First of all we note that $(Au|v)_H=(u|Av)_H$ for all $u,v \in \Dom{A}$ by the
Green's formula eq. (\ref{Ainf_eq_Green}) and therefore, since $A$ is densely
defined by lemma \ref{opth_lem_A0dense}, $A$ is symmetric.
Hence, it remains to show that $A^* \subset A$.

The relation $A_0 \subset A \subset A_1$ together with lemmas
\ref{opth_lem_adjA0} and \ref{opth_lem_adjA1} imply 
$A_1=A_0^* \supset A^* \supset A_1^*=A_0$.
Let $v \in \Dom{A^*} \subset \Dom{A_1}$.
By definition we have $(Au|v)_H=(u|A^*v)_H=(u|A_1v)_H$ for all $u \in \Dom{A}$.
On the other hand, according to the Green's formula eq. (\ref{Ainf_eq_Green}), 
we observe that $(Au|v)_H=[u,v]_p(b)-[u,v]_p(a)+(u|A_1v)_H$ for all $u \in
\Dom{A}$ which yields $[u,v]_p(b)-[u,v]_p(a)=0$ for all $u \in \Dom{A}$.
However, since $A$ is regular we can choose $(pu')(a)$ and $(pu')(b)$
arbitrarily which yields $v(a)=v(b)=0$.
Thus, $v \in \Dom{A}$ and therefore we have $A^* \subset A$.
\end{proof}

\subsection{Singular Sturm--Liouville Operators}
The results of the previous section are not very useful for concrete 
applications since most of the interesting Sturm--Liouville problems are
singular.
Thus, we have to generalize the theory to the singular case, i.e. in the sequel
we merely
assume $1/p,q,w \in L^1_\mathrm{loc}(a,b)$.

\paragraph{An auxiliary operator}
We define an auxiliary operator $\tilde{A}_0: \Dom{\tilde{A}_0}
\subset H \to H$ by 
$$ \Dom{\tilde{A}_0}:=\{u \in \Dom{A_1}: u \mbox{ has compact support}\}$$ 
and $\tilde{A}_0 u:=\alpha u$
for $u \in \Dom{\tilde{A}_0}$.

\paragraph{Regularized operators}
The main idea is to restrict the problem to a fixed interval 
$I:=[c,d] \subset (a,b)$ where everything is regular and then use the fact that
$I$ is arbitrary.
We define $H^I:=L^2_w(c,d)$.
Consider the mapping $i: H^I \to H$, $u \mapsto i(u)$ defined by
$$ (i(u))(x):=\left \{ \begin{array}{l} u(x) \mbox{ if }x \in [c,d] \\
0 \mbox{ if } x \in (a,b)\backslash [c,d] \end{array} \right. $$
Since $i: H^I \to H$ is injective we can identify $u$ with $i(u)$
and in this sense we have the inclusion $H^I \subset H$.
We define the regular operators $A^I_0$ and $A^I_1$ on $H^I$ analogous to 
$A_0$ and $A_1$ where $(a,b)$ is substituted by $(c,d)$.
According to the results of the previous section we have $(A_0^I)^*=A_1^I$ and
$(A_1^I)^*=A_0^I$.
Note further that $u \in \Dom{A_0^I}$ implies $i(u) \in \Dom{\tilde{A}_0}$ and
hence, we have $\Dom{A_0^I} \subset \Dom{\tilde{A}_0}$ in the same sense as $H^I
\subset H$.

\paragraph{Density of $\tilde{A}_0$}
We show that $\Dom{\tilde{A}_0}$ is dense in $H$.

\begin{lemma}
\label{opth_lem_tildeA0dense}
The operator $\tilde{A}_0$ is densely defined.
\end{lemma}

\begin{proof}
Let $f \in H$ with $(u|f)_H=0$ for all $u \in \Dom{\tilde{A}_0}$.
Since $\Dom{A_0^I} \subset \Dom{\tilde{A}_0}$ it follows that $(u|f)_H=0$ for
all $\Dom{A_0^I}$ and we can substitute the inner product on $H$ by the inner
product on $H^I$ which yields $(u|f|_I)_{H^I}=0$ for all $u \in \Dom{A_0^I}$.
Since $A_0^I: \Dom{A_0^I} \subset H^I \to H^I$ is densely defined by
lemma \ref{opth_lem_A0dense} we conclude that $f|_I=0$.
However, $I$ was arbitrary and therefore we infer that $f=0$ almost
everywhere.
\end{proof}

Lemma \ref{opth_lem_tildeA0dense} together with $(\tilde{A}_0
u|v)_H=(u|\tilde{A}_0v)_H=0$ for all $u,v \in \Dom{\tilde{A}_0}$ imply that
$\tilde{A}_0$ is symmetric.
Furthermore, since $\tilde{A}_0 \subset A_0 \subset A_1$, we observe that $A_0$
and $A_1$ are densely defined as well.

\paragraph{The equation $\alpha u=f$}
We consider the inhomogeneous equation $\alpha u=f$.

\begin{lemma}
\label{opth_lem_auf}
Let $f \in H$. Then, there exists a $u \in AC_\mathrm{loc}(a,b)$ with $pu' \in
AC_\mathrm{loc}(a,b)$ satisfying
$\alpha u=f$.
\end{lemma}

\begin{proof}
According to theorem \ref{opth_thm_ivp} there exist two linearly independent
functions $u_1,u_2 \in AC_\mathrm{loc}(a,b)$ with 
$pu_j' \in AC_\mathrm{loc}(a,b)$ satisfying $\alpha u_j=0$ ($j=1,2$).
Without loss of generality we can assume $[u_1,u_2]_p(x)=1$ (Green's formula eq.
(\ref{Ainf_eq_Green})).
We define $u$ by
\begin{multline*}
u(x):=c_1u_1(x)+c_2u_2(x)+u_1(x) \int_{x_1}^x u_2(s)f(s)w(s)ds
\\ -u_2(x) \int_{x_2}^x
u_1(s)f(s)w(s)ds 
\end{multline*}
where the constants $c_1,c_2 \in \mathbb{C}$ and $x_1,x_2 \in (a,b)$ can be
chosen arbitrarily.
A direct computation shows that $u,pu' \in AC_\mathrm{loc}(a,b)$ and 
$\alpha u=f$.
\end{proof}   

\paragraph{The adjoint operator}
Since $\tilde{A}_0$ is densely defined by lemma \ref{opth_lem_tildeA0dense}, the
adjoint $\tilde{A}_0^*$ is defined.

\begin{lemma}
\label{opth_lem_adjtildeA0}
The operator $A_1$ is the adjoint of $\tilde{A_0}$, i.e. $\tilde{A}_0^*=A_1$.
\end{lemma}

\begin{proof}
According to the Green's formula eq. (\ref{Ainf_eq_Green}) we have
$(\tilde{A}_0u|v)_H=(u|A_1v)_H$ for all $u \in \Dom{\tilde{A}_0}$ and all $v \in
\Dom{A_1}$ which means that $A_1$ is adjoint to $\tilde{A}_0$, i.e. $A_1 \subset
\tilde{A}_0^*$.
Thus, it suffices to show that $A_1 \supset \tilde{A}_0^*$.
Let $v \in \Dom{\tilde{A}_0^*}$, i.e. there exists an $f \in H$ such that 
$(\tilde{A}_0u|v)_H=(u|f)_H$ for all $u \in \Dom{\tilde{A}_0}$.
In particular it follows that $(\tilde{A}_0u|v)_H=(u|f)_H$ for all $u \in
\Dom{A_0^I}$ since $\Dom{A_0^I} \subset \Dom{\tilde{A}_0}$.
Invoking lemma \ref{opth_lem_auf} we find a $\tilde{v} \in AC_\mathrm{loc}(a,b)$
satisfying $\alpha \tilde{v}=f$.
Hence, we have
$(\tilde{A}_0u|v)_H=(u|f)_H=(u|\alpha \tilde{v})_H
=(u|\alpha \tilde{v}|_I)_{H^I}=(u|A_1^I
\tilde{v}|_I)_{H^I}=(A_0^Iu|\tilde{v}|_I)_{H^I}$ for all $u \in \Dom{A_0^I}$.
On the other hand we can write $(\tilde{A}_0u|v)_H=(A_0^I u|v)_{H^I}$ 
for all $u
\in \Dom{A_0^I}$.
This yields $(A_0^Iu|(v-\tilde{v})|_I)_{H^I}=0$ for all $u \in \Dom{A_0^I}$
which shows that $(v-\tilde{v})|_I \in (\im{A_0^I})^\perp=\ker{A_1^I}$.
Thus, $\alpha (v-\tilde{v})|_I=0$ which implies $\alpha v|_I=f|_I$.
Since this relation holds for all $I=[c,d] \subset (a,b)$ we infer 
$\alpha v=f \in H$.
Hence, we have $v,pv' \in AC_\mathrm{loc}(a,b)$ and $v, \alpha v \in H$ 
which shows
that $v \in \Dom{A_1}$.
Therefore, we have shown that $\tilde{A}_0^* \subset A_1$ and we are done.
\end{proof} 

\paragraph{A special case}
We consider the special case of a singular Sturm--Liouville operator on $(a,b)$ 
where $a$ is limit--circle and $b$ is limit--point.
The question is what kind of boundary condition one can choose 
in order to construct a self--adjoint
operator.

\begin{lemma}
\label{opth_lem_Aselfadj}
Suppose $a$ is in the limit--circle case and $b$ in the limit--point case.
Fix a $\chi \in \Dom{A_1}$ such that there exists a $v \in \Dom{A_1}$ with
$[v,\chi]_p(a) \not=0$ (such a $\chi$ exists since $a$ is limit--circle) 
and define $\Dom{A}:=\{u \in \Dom{A_1}:
[u,\chi]_p(a)=0\}$, $Au:=\alpha u$ for $u \in \Dom{A}$.
Then, the operator $A: \Dom{A} \subset H \to H$ is self--adjoint.
\end{lemma}

\begin{proof}
For $u_1,u_2,u_3,u_4 \in \Dom{A_1}$ we have the so--called \emph{Pl\"ucker 
identity}
$$
[u_1,u_2]_p(x)[u_3,u_4]_p(x)+[u_1,u_3]_p(x)[u_4,u_2]_p(x)
+[u_1,u_4]_p(x)[u_2,u_3]_p(x)=0. $$
Thus, choosing $u_1,u_2 \in \Dom{A}$, $u_3:=\chi$ and $u_4$ such that
$[\chi,u_4]_p(a)\not=0$ we obtain $[u_1,u_2]_p(a)=0$ for all $u_1,u_2 \in
\Dom{A}$.
Hence, the operator $A$ is symmetric ($b$ is limit--point) 
and it remains to show that $A^* \subset A$.

We have $\tilde{A}_0 \subset A$ which implies $A_1=\tilde{A}_0^*
\supset A^*$ by lemma \ref{opth_lem_adjtildeA0}.
Let $v \in \Dom{A^*} \subset \Dom{A_1}$.
By definition we have $(Au|v)_H=(u|A^*v)_H=(u|A_1v)_H$ for all $u \in \Dom{A}$.
Thus, the Green's formula yields $[u,v]_p(a)=0$ for all $u \in \Dom{A}$.
Note that $\chi \in \Dom{A}$ by definition and hence, the above formula with
$u=\chi$ yields $[\chi,v]_p(a)=0$ which shows that $v \in \Dom{A}$.
Therefore, we have $A^* \subset A$.
\end{proof}


==> wavemaps/cauchy.tex <==
\section{The Cauchy Problem}
We formulate the wave map equation (\ref{wm_eq_wm}) as an initial boundary 
value problem.

\subsection{Solutions of the Wave Map Problem}
We are looking for solutions of the wave map problem (\ref{wm_eq_wm}).
The fact that eq. (\ref{wm_eq_wm}) is a semilinear wave equation suggests the
formulation as an initial boundary value problem, i.e. we interpret eq.
(\ref{wm_eq_wm}) as a time evolution equation.
But what kind of initial values and boundary conditions are physically or
mathematically meaningful? 
In order to obtain a reasonable formulation, we require the following property:
Given initial data at a time $t=0$, there exists a unique 
solution (at least for small $t>0$) which satisfies the initial conditions 
and, additionally, certain regularity conditions.  
Based on physical considerations we expect that prescribing  
$\psi(0, \cdot)$ and $\psi_t(0, \cdot)$ as initial data is the only reasonable
choice.
The boundary conditions are suggested by regularity assumptions.

In the previous sections we have assumed the function $\psi$ 
to be smooth.
However, from the point of view of hyperbolic partial differential equations
this seems to be unnecessarily restrictive.
Therefore, we will weaken the assumption of smoothness in our further 
discussion.
Nevertheless, we will not formulate precise regularity conditions at this stage
because this is a very subtle question and hence we will postpone it.
However, as a minimal assumption we require the function $\psi$ to be
continuous.
Moreover, we assume that that the second derivatives of $\psi$ are well-behaved
in a sense which will be made precise below. 
By construction, $\psi$ is defined on $(0,\infty)$ and has range in $(0, \pi)$.
However, for physical reasons we require $\psi$ to be continuously extendible to
$r=0$ which corresponds to the origin of Minkowski space.
Hence, we define $\psi(t,0):=\lim_{r \to 0} \psi(t,r)$ and assume the 
regularity condition $\sin(2 \psi(t,0))=0$
which yields the three possibilities $\psi(t,0)=0, \frac{\pi}{2} \mbox{ or }
\pi$ for all $t$.
However, without loss of generality the third case $\psi(t,0)=\pi$ can be left
out since $\psi+\pi$ is a solution of eq. (\ref{wm_eq_wm}) if and only if $\psi$
is.

Another restriction emerges from energy considerations as will be discussed in
the next section. 

\subsection{Energy Conservation}
We define the Lagrangian $\mathcal{L}$ by 
$$ \mathcal{L}(\psi, \psi_t, \psi_r, r):=
\psi_t^2-\psi_r^2-2\frac{\sin^2(\psi)}{r^2}. $$
As we have seen, the wave map equation (\ref{wm_eq_wm}) is derived from the
action functional
$$ \psi \mapsto \int_{-\infty}^\infty \int_0^\infty \mathcal{L} dr dt. $$
Since $\mathcal{L}$ does not depend on $t$ explicitly, there is a conserved
quantity according to Noether's theorem (cf. \cite{Shatah1998}).
The \emph{energy density} is given by
$$ \frac{\partial \mathcal{L}}{\partial
\psi_t}\psi_t-\mathcal{L} =\psi_t^2+\psi_r^2+
\frac{2 \sin^2(\psi)}{r^2}. $$
Then, the \emph{energy} $E$ is defined by
\begin{equation}
\label{wm_eq_E}
E(\psi(t, \cdot)):=\int_0^\infty \left ( \psi_t^2(t,r)+\psi_r^2(t,r)+
\frac{2 \sin^2(\psi)}{r^2} \right ) r^2 dr. 
\end{equation}
The function $t \mapsto E(\psi(t,\cdot))$ is constant if $\psi$ is a smooth
solution of eq. (\ref{wm_eq_wm}) having compact spatial support, i.e.
$\psi(t,\cdot) \in C^\infty_c(0,\infty)$ for all $t$.
This can easily be verified by differentiating $t \mapsto E(\psi(t,\cdot))$ 
and integration by parts.
However, the same is true under weaker assumptions.
It is sufficient to require finiteness of $E(\psi(t,\cdot))$.
We will discuss this issue later on in connection with Sobolev spaces. 

\subsection{Formulation of the Cauchy problem}
For physical reasons we are only interested in finite energy solutions of eq.
(\ref{wm_eq_wm}) and we restrict ourselves to the boundary condition
$\psi(t,0)=0$ for all $t$.
Therefore, we can formulate the problem we intend to study in a symbolic way 
as follows.
Find suitable function spaces $X_1$, $X_2$ such that for
prescribed initial data $f \in X_1$, $g \in X_2$ there exists a $T>0$ 
and a unique solution $\psi$ of
$$ \psi_{tt} - \psi_{rr} -\frac{2}{r} \psi_r + \frac{\sin(2 \psi)}{r^2}=0 $$
which satisfies $\psi(t,0)=0$, $E(\psi(t,\cdot)) < \infty$ for all $t \in
[0,T]$
and 
$\psi(0, \cdot)=f$,  $\psi_t(0, \cdot)=g$.

In order to give a precise formulation of the problem, we choose an operator
theoretic approach. 
This treatment is based on the observation that partial differential equations
can be interpreted as ordinary differential equations on Banach spaces.
However, to formulate the problem in this elegant abstract setting we need some
mathematical preparation.


==> wp/linwm.tex <==
\section{The Linearized Wave Map Problem}
\label{linwm_sec}
Using the semigroup techniques developed in the last section we show
well--posedness of the linearization of the wave map equation
(\ref{wm_eq_wm})
$$
\psi_{tt} - \psi_{rr} -\frac{2}{r} \psi_r + \frac{\sin(2 \psi)}{r^2}=0.
$$
We rewrite eq. (\ref{wm_eq_wm}) as
$$ \psi_{tt} = \psi_{rr} + \frac{2}{r} \psi_r -\frac{2}{r^2} \psi +F(\psi) $$
where 
$$ F(\psi):=\frac{2\psi-\sin(2 \psi)}{r^2} $$
and consider the linear evolution equation
\begin{equation}
\label{linwm_eq_linwm}
\left \{ \begin{array}{l}
\psi_{tt} = \psi_{rr} + \frac{2}{r} \psi_r -\frac{2}{r^2}
\psi \\
\psi(0,r)=\psi_0(r), \psi_t(0,r)=\psi_1(r) \end{array} \right. 
\end{equation}
For simplicity we will restrict ourselves to Dirichlet boundary conditions.

\subsection{Operator Formulation}
First we informally discuss how to "guess" the right function space for an
appropriate operator formulation of eq. (\ref{linwm_eq_linwm}).
We intend to find an operator $B$ such that \footnote{We remark that there is
a slightly different approach which is more elegant. It relies on the concept of
the square root of a nonnegative self--similar operator.
However, the introduction of these concepts requires
some effort and hence we have avoided it at this stage
and choose a more elementary approach instead.} 
$$ -(B^*B)u(r)=u''(r)+\frac{2}{r}u'(r)-\frac{2}{r^2}u(r). $$
Hence, we have to choose the Hilbert space $H$ in such a way that the above
differential operator becomes symmetric since $-B^*B$ is symmetric.
This motivates the choice 
$H:=L^2_w(r_1,r_2)$ where $r_1, r_2 \in [0,\infty)$, $r_1<r_2$ and $w(r):=r^2$.
However, in order to make the operator symmetric with respect to the inner
product on $H$ the functions it is applied to
have to satisfy certain boundary conditions.
This requirement motivates the choice of the domain $\Dom{B}$ below.
Now we give the precise derivation.

Consider the weighted Sobolev space 
$H^1_{(2,w)}(r_1,r_2)$ (the factor $2$ as
a weight is introduced for convenience only).
The following lemma shows that functions in $H^1_{(2,w)}(r_1,r_2)$ are 
continuous.

\begin{lemma}
\label{linwm_lem_estC}
We have the embedding $H^1_{(2,w)}(r_1,r_2) \hookrightarrow C[b,r_2]$ for any
$b \in (r_1,r_2)$.
\end{lemma} 

\begin{proof}
Let $u \in H^1_{(2,w)}$. We write
$$ ru(r)=au(a)+\int_a^r u(s)ds + \int_a^r su'(s)ds $$
for any $a \in [r_1,r_2]$.
Integration and application of the Cauchy-Schwarz inequality yield
$$ R|au(a)| \leq \int_{r_1}^{r_2} |ru(r)|dr + R\int_{r_1}^{r_2} |u(r)|dr + 
R \int_{r_1}^{r_2} |ru'(r)|dr 
 \leq C \|u\|_{H^1_{(2,w)}(r_1,r_2)}
$$
where $R:=r_2-r_1$ and $C>0$ is a constant which depends on $r_1$ and $r_2$ 
only.
Hence, for any $b \in (r_1,r_2)$ we have
$$ \sup_{a \in [b,r_2]} |u(a)| \leq \frac{C}{bR} \|u\|_{H^1_{(2,w)}(r_1,r_2)} 
$$ 
which implies the claim.
\end{proof}

\begin{remark}
\label{linwm_rem_DBC}
If $r_1>0$ then we can even choose $b=r_1$ and hence, we have
$H^1_{(2,w)}(r_1,r_2) \hookrightarrow C[r_1,r_2]$.
\end{remark}

We set $\Dom{B}:=\{u \in H^1_{(2,w)}(r_1,r_2): u(r_1)=u(r_2)=0\}$ if $r_1>0$ and
$\Dom{B}:=\{u \in H^1_{(2,w)}(r_1,r_2): u(r_2)=0\}$ if $r_1=0$.
These definitions make sense thanks to lemma \ref{linwm_lem_estC}. 
We define 
$B: \Dom{B} \subset H \to H$ by
$(Bu)(r):=-u'(r)-\frac{2}{r}u(r)$.
Then, $B$ is a densely defined linear operator on $H$.

\begin{lemma}
\label{linwm_lem_DBBanach}
$\left( \Dom{B}, \|\cdot\|_{H^1_{(2,w)}(r_1,r_2)} \right )$ is a Banach space.
\end{lemma} 

\begin{proof}
Let $(u_j) \subset \Dom{B}$ be a sequence with $u_j \to u$ in 
$H^1_{(2,w)}(r_1,r_2)$.
Then, by lemma \ref{linwm_lem_estC}, $u_j(r_2) \to u(r_2)$.
From this it follows that $u(r_2)=0$ since $u_j(r_2)=0$ for all $j \in
\mathbb{N}$.
The same holds true for $u(r_1)$ if $r_1>0$.
Hence, $\Dom{B}$ is a closed subspace of the Banach space 
$H^1_{(2,w)}(r_1,r_2)$
and therefore, $\left (\Dom{B}, \|\cdot\|_{H^1_{(2,w)}(r_1,r_2)} \right)$ 
is a Banach space
itself.
\end{proof}

\begin{lemma}
\label{linwm_lem_Bclosed}
The operator $B$ is closed.
\end{lemma}

\begin{proof}
We show that $(\Dom{B}, \|\cdot\|_B)$ is a Banach space which is equivalent to
$B$ being closed.

Let $u \in \Dom{B}$. Integration by parts shows that
$$ \|Bu\|_H^2=(Bu|Bu)_H=\int_{r_1}^{r_2} r^2 |u'(r)|^2 + 2 \int_{r_1}^{r_2}
|u(r)|^2 dr $$
and hence, $\|Bu\|_H=\|u\|_{H^1_{(2,w)}(r_1,r_2)}$.
This shows $\|u\|_B^2=\|Bu\|_H^2 + \|u\|_H^2 \geq \|u\|_{H^1_{(2,w)}(r_1,r_2)}$.
Moreover, since $\|u\|_{L^2(r_1,r_2)} \geq C\|u\|_H$ for a $C>0$, we see that
there exists a constant $C>0$ such that $\|u\|_B \leq
C\|u\|_{H^1_{(2,w)}(r_1,r_2)}$.
Hence, the norms $\|\cdot\|_B$ and $\|\cdot\|_{H^1_{(2,w)}(r_1,r_2)}$ are
equivalent which shows that $(\Dom{B}, \|\cdot\|_B)$ is a Banach space.
\end{proof}

\begin{corollary}
There exists a constant $\gamma>0$ such that the operator $B$ satisfies 
$(Bu|Bu)_H \geq \gamma(u|u)_H$ for all $u \in \Dom{B}$.
\end{corollary}

\begin{proof}
This follows immediately from the proof of lemma \ref{linwm_lem_Bclosed}.
\end{proof} 

Hence, invoking theorem \ref{cauchy_thm_gen} we see that the associated
first--order Cauchy problem is well--posed.
The next lemma connects this result to the problem eq.
(\ref{linwm_eq_linwm}), i.e. we show that
\begin{equation}
\label{linwm_eq_linwmop} \left \{ \begin{array}{l} \psi_{tt}(t)=-B^*B\psi(t) \mbox{ for } t>0 \\
\psi(0)=\psi_0, \psi_t(0)=\psi_1 \end{array} \right .
\end{equation}
is an operator version of eq. (\ref{linwm_eq_linwm}).

\begin{lemma}
\label{linwm_lem_B}
Let $u \in C^\infty_c(r_1,r_2)$. Then,
$$ (-B^*Bu)(r)=u''(r)+\frac{2}{r}u'(r)-\frac{2}{r^2}u(r).$$
\end{lemma}

\begin{proof}
We set $\Dom{C}:=C^\infty_c(r_1,r_2)$ and define $C: \Dom{C} \subset H \to H$ by
$Cu:=u'$ for $u \in \Dom{C}$.
Integration by parts shows that $(Bu|v)_H=(u|Cv)_H$ for all $u \in \Dom{B}$ and
$v \in \Dom{C}$.
Thus, $C$ is adjoint to $B$, i.e. $C \subset B^*$.
Hence, for $u \in C^\infty_c(r_1,r_2)$ we calculate
$$ (-B^*Bu)(r)=(-CBu)(r)=\frac{d}{dr} \left (u'(r)+\frac{2}{r}u(r) \right
)=u''(r)+\frac{2}{r}u'(r)-\frac{2}{r^2}u(r). $$
\end{proof}

Hence, for smooth functions with compact support, the operator version eq.
(\ref{linwm_eq_linwmop}) is equivalent to eq. (\ref{linwm_eq_linwm}).
However, the generation result is more general.
It states well--posedness for $(\psi, \psi_t) \in \Dom{B} \times H$.
The generation theorem \ref{cauchy_thm_gen} does not only yield
well--posedness,
it provides the framework for a proper formulation of the
problem.
Hence, we will say that an informal problem like eq. (\ref{linwm_eq_linwm}) is
\emph{well--posed} if one can construct a well--posed operator version associated
to it.

\paragraph{Estimates}
The generated semigroup satisfies the estimate $\|S(t)\|_{\mathcal{B}(X)} \leq
1$ where $X=\Dom{B} \times H$ by theorem \ref{cauchy_thm_gen}.
For the Cauchy problem eq. (\ref{linwm_eq_linwm}) this means that a solution
$\psi$ can be estimated in terms of the initial data by
$$ \int_{r_1}^{r_2} (r^2 \psi_t^2(t,r)+r^2 \psi_r^2(t,r)+2\psi^2(t,r))dr $$
$$\leq \int_{r_1}^{r_2}
(r^2 \psi_t^2(0,r)+r^2 \psi_r^2(0,r)+2\psi^2(0,r))dr $$
(we assume $\psi$ to be real).
However, this result is not so surprising since 
$$ t \mapsto \int_{r_1}^{r_2} (r^2 \psi_t^2(t,r)+r^2 \psi_r^2(t,r)+2\psi^2(t,r))dr $$
is the conserved energy of the problem eq. (\ref{linwm_eq_linwm}) for 
$(t,r) \in
[0,\infty) \times [r_1,r_2]$ if one
imposes the condition $\psi(t,r_2)=0$ and, if $r_1>0$, 
$\psi(t,r_1)=0$ for all $t \geq 0$.
Thus, the semigroup approach we have taken leads to a very physical formulation
of the problem since the underlying norm coincides with the conserved energy.


==> wpwm/linwm.tex <==
\section{The Linearized Wave Map Problem}
\label{linwm_sec}
Using the semigroup techniques developed in the last section we show
well--posedness of the linearization of the wave map equation
(\ref{wpwm_eq_wm}).
We rewrite eq. (\ref{wpwm_eq_wm}) as
$$ \psi_{tt} = \psi_{rr} + \frac{2}{r} \psi_r -\frac{2}{r^2} \psi +F(\psi) $$
where 
$$ F(\psi):=\frac{2\psi-\sin(2 \psi)}{r^2} $$
and consider the linear evolution equation
\begin{equation}
\label{linwm_eq_linwm}
\left \{ \begin{array}{l}
\psi_{tt} = \psi_{rr} + \frac{2}{r} \psi_r -\frac{2}{r^2}
\psi \\
\psi(0,r)=\psi_0(r), \psi_t(0,r)=\psi_1(r) \end{array} \right. 
\end{equation}

\subsection{The Operator $A$}
Consider the \emph{formal differential expression} $a$ defined by
$$ a:=\frac{1}{r^2}\left ( -\frac{d}{dr}r^2 \frac{d}{dr}+2 \right ). $$
The linearized wave map equation can be written as
$\psi_{tt}=-a\psi$.
$a$ is in Sturm--Liouville form where $p(r)=r^2$, $q(r) \equiv 2$ and
$w(r)=r^2$.

\paragraph{Definition of the operator}
We intend to construct a self--adjoint operator generated by $a$.
Thus, we choose $H:=L^2_w(0,\infty)$.
Consider the equation $au=0$, explicitly given by
$$ u''+\frac{2}{r}u'-\frac{2}{r^2}u=0. $$
This equation has the two linearly independent solutions $u_0(r)=r$ and
$u_\infty(r)=\frac{1}{r^2}$.
The solution $u_0$ does not belong to $H$ near $\infty$, while $u_\infty$ 
does not
belong to $H$ near $0$.
Thus, according to the results of sec. \ref{sl_sec}, we conclude that both
endpoints $0$ and $\infty$ are in the limit--point case.
We define $\Dom{A}:=\{u \in H: u,pu' \in AC_\mathrm{loc}(0,\infty), au \in H\}$,
$Au:=au$ for $u \in \Dom{A}$.
Then, the operator $A: \Dom{A} \subset H \to H$ is self--adjoint (Lemma
\ref{sl_lem_lplp}).

\paragraph{Properties of $A$}
Consider the operator $\tilde{A}_0: \Dom{\tilde{A}_0}\subset H \to H$ 
defined by $\Dom{\tilde{A}_0}:=\{u
\in \Dom{A}: u \mbox{ has compact support}\}$ and $\tilde{A}_0u:=au$ for
$u \in \Dom{\tilde{A}_0}$.
In sec. \ref{sl_sec} we have shown that $A$ is the closure of $\tilde{A}_0$.
Thus, $\Dom{\tilde{A}_0}$ is a core for $A$.
Integration by parts yields
$$ \int_0^\infty (\tilde{A}_0 u)(r)\overline{u(r)}w(r)dr=\int_0^\infty
p(r)|u'(r)|^2w(r)dr+2\int_0^\infty |u(r)|^2 dr \geq 0 $$
for all $u \in \Dom{\tilde{A}_0}$ which shows that $(\tilde{A}_0u|u)_H \geq 0$.
Let $u \in \Dom{A}$. Then, since $\Dom{\tilde{A}_0}$ is a core for $A$, 
there exists a
sequence $(u_j) \subset \Dom{\tilde{A}_0}$ such that $u_j \to u$ in 
$H$ and $\tilde{A}_0u_j \to
Au$ in $H$.
Hence, the inequality $(\tilde{A}_0u_j|u_j)_H \geq 0$ remains valid in the 
limit and we
conclude that $(Au|u)_H \geq 0$ for all $u \in \Dom{A}$.

\subsection{Well--Posedness}
Since $A$ is nonnegative, the square root $A^{1/2}$ exists.
We define $X:=\Dom{A^{1/2}} \times H$ and
$\|(u,v)\|_X^2:=\|u\|_{A^{1/2}}^2+\|v\|_H^2$ for $(u,v) \in X$.
Furthermore, we set $\Dom{L}:=\Dom{A} \times \Dom{A^{1/2}}$ and
$L(u,v):=(v,-Au)$ for $(u,v) \in \Dom{L}$.
Consider the evolution equation
$$ \left \{ \begin{array}{l} \frac{d}{dt} \mathbf{u}(t)=L\mathbf{u}(t) \mbox{
for } t>0 \\
\mathbf{u}(0)=\mathbf{u_0} \end{array} \right . $$
for $\mathbf{u_0} \in X$ which is an operator formulation of the linearized wave
map problem eq. (\ref{linwm_eq_linwm}).
Invoking Theorem \ref{gamma0_thm_gen} we immediately obtain well--posedness.
Theorem \ref{gamma0_thm_gen} also yields conservation of energy for 
solutions of the linearized wave map problem:
If $\mathbf{u}(t)=:(u(t),v(t))$ is a solution then
its conserved energy is given by $\|A^{1/2}u(t)\|_H^2+\|v(t)\|_H^2$.

Thus, with the abstract theory at hand it is very easy to obtain a
well--posedness result for a linear wave equation of that type.


